Where Will Players Move Next? Dynamic Graphs and Hierarchical Fusion for Movement Forecasting in Badminton

Sports analytics has captured increasing attention since analysis of the various data enables insights for training strategies, player evaluation, etc. In this paper, we focus on predicting what types of returning strokes will be made, and where players will move to based on previous strokes. As this problem has not been addressed to date, movement forecasting can be tackled through sequence-based and graph-based models by formulating as a sequence prediction task. However, existing sequence-based models neglect the effects of interactions between players, and graph-based models still suffer from multifaceted perspectives on the next movement. Moreover, there is no existing work on representing strategic relations among players' shot types and movements. To address these challenges, we first introduce the procedure of the Player Movements (PM) graph to exploit the structural movements of players with strategic relations. Based on the PM graph, we propose a novel Dynamic Graphs and Hierarchical Fusion for Movement Forecasting model (DyMF) with interaction style extractors to capture the mutual interactions of players themselves and between both players within a rally, and dynamic players' tactics across time. In addition, hierarchical fusion modules are designed to incorporate the style influence of both players and rally interactions. Extensive experiments show that our model empirically outperforms both sequence- and graph-based methods and demonstrate the practical usage of movement forecasting.

==> sections/2-related-work.tex <==
\section{Related Work}
\label{sec:related-work}

Sports analytics aims at applying data-driven methods to a wide variety of sources of sports data for gaining insights and tactics of teams and players.
The applications of sports analytics can be mainly divided into two categories: on-field analytics and off-field analytics.
On-field analytics focuses on improving the performance of a team or individual player by providing objective perspectives such as the fitness of players \cite{rydzik2021physical, ramirez2021effects}, player performance \cite{Wang2020badminton,jamil2021using,terner2021modeling}, and the potential rising stars \cite{DBLP:journals/kbs/MahmoodDA21}. 
On the other hand, off-field analytics assists team owners in increasing profits by studying the relationship with fans \cite{paek2021examining, yim2021identifying, qian2022watching}, and their marketing strategies \cite{melton2021examining, richelieu2021strategic}.
In this paper, we focus on on-field analytics for investigating the performance of players.
% which has been analyzed by deep learning algorithms for modeling various aspects \cite{DBLP:conf/kdd/MerhejBMR21,DBLP:conf/kdd/WangDXSHCZZZW21}.
Generally, \citet{DBLP:conf/ijcai/DecroosBHD20} presents five main issues around artificial intelligence in sports analytics:
representation, interpretability, decision making, understanding behavior, and experimental evaluation.
In badminton, there are few applications tackling these issues.
% \citet{Wang2020badminton} constructed an analysis pipeline that transforms videos into data on the visualization platform to provide objective perspectives to find opponents' weaknesses and develop tactics.
\citet{DBLP:conf/icdm/WangCYWFP21,10.1145/3551391} formalized the badminton language for describing the process of a rally , which can be used for our inputs and outputs of movement forecasting (i.e., players, shot types, and locations).
ShuttleNet is proposed for stroke forecasting to simulate players' strategies based on the past information \cite{DBLP:conf/aaai/WangSCP22}.
Our work introduces another instrumental but challenging application by predicting the next movements and the shot type of both players in a rally, which helps players investigate the effect and behavior of each movement\footnote{More related work is discussed in Appendix C.}.
% Existing works related to movements on the court in badminton only utilize statistical inference to analyze the relationship between movements in different rounds \cite{josue2020movement,valldecabres2020players}, which can not simulate movements on the court.

==> tables/match-info.tex <==
\begin{tabular}{cccc}
    \toprule
    Tournament & Round \\
    \midrule
    Fuzhou Open 2018 & Finals \\
    Denmark Open 2018 & Finals \\
    Malaysia Open 2018 & Quarter-finals \\
    Asia Championships 2018 & Quarter-finals \\
    Fuzhou Open 2019 & Semi-finals \\
    Fuzhou Open 2019 & Finals \\
    Hong Kong Open 2019 & Quarter-finals \\
    World Tour Finals & Group-Stage \\
    Korea Open 2019 & Finals \\
    Denmark Open 2019 & Quarter-finals \\
    China Open 2019 & Quarter-finals \\
    Indonesia Open 2019 & Finals \\
    World Tour Finals 2019 & Group-Stage \\
    World Tour Finals 2019 & Semi-finals \\
    World Tour Finals 2019 & Finals \\
    World Championships 2019 & Quarter-finals \\
    Denmark Open 2019 & Round-of-32 \\
    Sudirman Cup 2019 & Quarter-finals \\
    Sudirman Cup 2019 & Group-Stage \\
    Indonesia Open 2019 & Quarter-finals \\
    All England Open 2020 & Quarter-finals \\
    All England Open 2020 & Finals \\
    Thailand Masters 2020 & Semi-finals \\
    Indonesia Masters 2020 & Quarter-finals \\
    Indonesia Masters 2020 & Semi-finals \\
    Indonesia Masters 2020 & Finals \\
    Malaysia Masters 2020 & Round-of-16 \\
    Malaysia Masters 2020 & Quarter-finals \\
    Malaysia Masters 2020 & Semi-finals \\
    Malaysia Masters 2020 & Finals \\
    YONEX Thailand Open 2021 & Quarter-finals \\
    YONEX Thailand Open 2021 & Semi-finals \\
    YONEX Thailand Open 2021 & Finals \\
    TOYOTA Thailand Open 2021 & Quarter-finals \\
    TOYOTA Thailand Open 2021 & Semi-finals \\
    TOYOTA Thailand Open 2021 & Finals \\
    HSBC BWF World Tour Finals 2020 & Group-Stage \\
    HSBC BWF World Tour Finals 2020 & Quarter-finals \\
    HSBC BWF World Tour Finals 2020 & Semi-finals \\
    HSBC BWF World Tour Finals 2020 & Finals \\
    \bottomrule
\end{tabular}

==> tables/shot-type-descriptions.tex <==
\begin{tabular}{c|l}
    \toprule
    Shot type       & Description \\
    \midrule
    net shot        & A soft shot that places the shuttle close to the net.\\
    \midrule
    smash           & A fast, downward angled shot that is performed with an overhand motion. \\
    \midrule
    lob       & \makecell[l]{A defensive shot that is typically performed from the front of the court by pushing the shuttle high and \\ far to the back of the opponent’s end of the court.} \\
    \midrule
    clear & A high overhand shot where the player hits the shuttle from one end of the court to the other end. \\
    \midrule
    drive & \makecell[l]{A fast and flat shot that travels just above the net, which is used for both offensive and defensive \\ purposes.}\\
    \midrule
    drop & \makecell[l]{An active shot that places the shuttle close to the net, often in an attempt to make the opponent move or \\ to set up for the next shot.}\\
    \midrule
    push/rush       & A shot pushed/rushed from near the net to land at the back court for landing quickly.\\
    \midrule
    defensive shot  & A shot that returns the smash from the middle or back court of the opponent to the middle or back court. \\
    \midrule
    short service   & A serve that goes over the top of the net and lands near the short service line.\\
    \midrule
    long service    & A serve that goes high and deep into the opponent’s back court.\\
    \bottomrule
\end{tabular}
